Probing Turbulence in the Interstellar Medium using Radio-Interferometric Observations of Neutral Hydrogen

We develop a visibility based power spectrum estimator to probe the power spectrum directly from the interferometric observations and also estimate the errors in it. A numerical simulation of synthetic observations is also performed to access the efficacy and limitations of this estimator. We use this estimator to evaluate the power spectrum of three individual spiral galaxies, a dwarf galaxy sample and THINGS * spiral galaxies. In each case, the power spectrum is found to follow a power law PHI (U) = AU {\alpha} over a specific length scale range. The estimated value for the slope {\alpha} ranges from ~ ~1.5 to ~ -2.6 for the sample of dwarf galaxies. We interpret this bi-modality as arising due to 2D turbulence on length scales much larger than the scale-height of the galaxy disk and 3D otherwise. The power law slope also show a weak correlation with the surface density of star formation rate for these galaxies. We found for the external spiral galaxies the power spectrum is a power law up to a length scale of 10 to 16 kpc, indicating turbulence to be operational at these large length scales. We measure the scale-height of the external nearly face-on spiral galaxy NGC 1058 to be ~ 500 pc interpreting a change in the slope observed in it's power spectrum. Power spectrum of the harassed galaxy NGC 4254 is found to be affected by galaxy harassment. For 18 spiral galaxies derived from the THINGS sample we found no correlation between the power law slope and the different dynamical parameters of these galaxies. For most of the dwarf and spiral galaxies, the intensity fluctuation power spectrum is found to be a direct probe of the density fluctuation and not affected by the velocity fluctuations in ISM. We would attempt to understand these new observations in terms of physical models of the ISM in future.

==> abstract/abstract.tex <==

%\thispagestyle{empty}

%\pagenumbering{roman}

%\vspace{-0.5cm}
%\vspace{2cm}    %%%Parsun

\begin{center}
{\Large \bf Abstract}
\end{center}
%\vspace{.2cm}

\begin{singlespacing}


{\bf Keywords}:
\end{singlespacing}

%\newpage
\clearpage
%\setcounter{page}   %{26}     %%I have added this to adjust the page number

\thispagestyle{empty}

\newpage
%\newpage


==> chapter6/figure.tex <==
\begin{figure*}
\begin{center}
\epsfig{file=./chapter6/fig1.eps,width=5.6in}
\end{center}
\caption{}
\label{fig:fig1}
\end{figure*}

\begin{figure*}
\begin{center}
\epsfig{file=./chapter6/fig2.eps,width=5.6in, angle=0}
\end{center}
\caption{}
\label{fig:fig2}
\end{figure*}

\begin{figure*}
\begin{center}
\epsfig{file=./chapter6/fig3.eps,width=5.6in, angle=0}
\end{center}
\caption{}
\label{fig:fig3}
\end{figure*}

\begin{figure*}
\begin{center}
\epsfig{file=./chapter6/fig4.eps, angle=0, width=5.6in}
\end{center}
\caption{} 
\label{fig:fig4}
\end{figure*}

\begin{figure*}
\begin{center}
\epsfig{file=./chapter6/AHIS.eps, angle=-90, width=5.6in}
\end{center}
\caption{} 
\label{fig:hist}
\end{figure*}

\begin{figure*}
\begin{center}
\epsfig{file=./chapter6/IA.eps, angle=-90, width=2.6in}
\end{center}
\caption{} 
\label{fig:inc}
\end{figure*}

\begin{figure*}
\begin{center}
\epsfig{file=MDY.eps, angle=-90, width=2.6in}
\end{center}
\caption{} 
\label{fig:mdy}
\end{figure*}

\begin{figure*}
\begin{center}
\epsfig{file=MHI.eps, angle=-90, width=2.6in}
\end{center}
\caption{} 
\label{fig:mhi}
\end{figure*}

\begin{figure*}
\begin{center}
\epsfig{file=VDP.eps, angle=-90, width=2.6in}
\end{center}
\caption{} 
\label{fig:disp}
\end{figure*}


\begin{figure*}
\begin{center}
\epsfig{file=SFRO.eps,width=2.6in, angle=-90}
\epsfig{file=SFRR.eps,width=2.6in, angle=-90}
\end{center}
\caption{}
\label{fig:sfr}
\end{figure*}




==> chapter6/table.tex <==


\begin{table*}
\centering
\begin{tabular}{lcccccccc|}
\hline
Galaxy & & $\Delta \ v$ & $U_{min}$   & $U_{max}$     & $R_{min}$ & $R_{max}$ & $\alpha$ &\\
       & & $km\ s^{-1}$ & k $\lambda$ &  k $\lambda$ & kpc      & kpc & &  \\
\hline \hline  
NGC628   &   & 2.6 & 1.0 & 10.0 & 0.75 &  7.5 & -1.6+-0.1 & \\
NGC925	 &   & 2.6 & 1.0 & 10.0 & 0.92 &  9.2 & -1.0+-0.2 & \\
NGC2403	 & * & 5.2 & 0.7 & 7.0  & 0.6  &  4.0 & -2.1+-0.1 & \\
NGC2841N &   & 5.2 & 1.0 & 10.0 & 1.4  & 14.0 & -1.7+-0.2 & \\
NGC2841S &   & 5.2 & 1.0 & 10.0 & 1.4  & 14.0 & -1.5+-0.2 & \\
NGC2903	 &   & 5.2 & 0.8 & 8.0  & 1.1  & 11.1 & -1.5+-0.2 & \\
NGC2976	 &   &  -  & -   & -    &  -   &   -  &     -     & \\    
NGC3031N &   & 2.6 & 2.0 & 10.0 & 0.4  & 1.8  & -0.7+-0.1 & \\
NGC3031S &   &  -  & -   & -    &  -   &   -  &     -     & \\
NGC3184	 &   & 2.6 & 0.7 & 7.0  & 1.6  & 15.8 & -1.3+-0.2 & \\
NGC3198	 & * & 5.2 & 1.6 & 10.0 & 1.4  &  8.6 & -1.6+-0.3 & \\
NGC3351	 &   &  -  & -   & -    &  -   &   -  &     -     & \\	
NGC3521N &   & 5.2 & 1.0 & 17.0 & 0.63 & 10.7 & -1.6+-0.2 & \\
NGC3521S &   & 5.2 & 1.0 & 17.0 & 0.63 & 10.7 & -1.8+-0.1 & \\
NGC3621	 & * & 5.2 & 1.0 & 12.0 & 0.55 &  6.6 & -1.9+-0.2 & \\
NGC4736	 & * & 5.2 & 0.6 & 10.0 & 0.5  &  7.8 & -0.9+-0.2 & \\
NGC5055	 &   & 5.2 & 1.0 & 10.0 & 1.0  & 10.0 & -1.6+-0.1 & \\
NGC5194	 &   & 5.2 & 1.0 & 8.0  & 1.0  &  8.0 & -1.7+-0.2 & \\
NGC5236	 &   & 2.6 & 0.6 & 6.0  & 0.75 &  7.5 & -1.9+-0.2 & \\
NGC5457	 &   & 5.2 & 0.6 & 12.0 & 0.62 & 12.3 & -2.2+-0.1 & \\
NGC6946	 &   & 1.3 & 1.5 & 10.0 & 0.3  & 4.0  & -1.6+-0.1 & \\
NGC7331	 &   &  -  & -   & -    &  -   &   -  &     -     & \\    
NGC7793	 &   & 2.6 & 0.6 & 6.0  & 0.65 & 6.5  & -1.7+-0.2 & \\
\end{tabular}
\caption{The results for  the 8 galaxies in our sample.  Rows 1-6
  gives (1) $N$  the number of channels  averaged over, (2) the 
  corresponding  velocity width 
  (3) $\alpha$ the best fit slope for the HI power spectrum, 
  (4) $U$ range over which the power law fit is valid,  (5) length-scales
  over which the power law fit is valid  and (6) the
  goodness  of fit $\chi^2$ per degree of freedom. Row (7) Possible
  limits for the spectral slope of the velocity structure function.} 
\label{tab:result}
\end{table*}


==> dnt_delete/tst <==
$z$ & & Redshift\\
$M_0$&& Mass of Sun\\
$\tau_e$&& CMB electron scattering optical depth\\
$\ell$&&Angular mutipole\\
$\Delta \nu$&&Frequency separation between two channels\\
$T_{sky}$&& Sky brightness temperature\\
$R_b$&& Comoving radius of the ionized bubble\\
$x_{HI}$&& Neutral hydrogen fraction\\
${\bar x_{HI}}(z)$&& Spatially averaged neutral hydrogen fraction\\
${\bar I_{\nu}}$&& Average specific intensity of the redshifted HI\\
&&21-cm from the EoR\\
$T(\nu, {\hat n})$&& Excess 21-cm brightness temperature \\
&&observed at a frequency $\nu$ along a direction ${\hat n}$\\
${\bar T(z)}$&& Spatially average Excess 21-cm brightness\\
&&temperature at redshift $z$\\
$\eta_{HI}(z,{\hat n}r_{\nu})$&&21-cm radiation efficienct in redshift
space\\
$Y$&&Helium mass fraction\\
$C_l(\Delta \nu)$&& Multifrequency angular power spectrum\\
$\delta_{HI}(z,{\hat n}r_{\nu})$&& Fluctuations in neutral hydrogen
density field\\
$T_{\gamma}$&&CMB temperature\\
$T_s$&& Spin temperature of hydrogen gas\\
$v(z,{\hat n}r_{\nu})$&&peculiar velocity of neutral hydrogen gas\\
$\Delta_{HI}(z,{\bf k})$
\end{tabular}
\end{center}



==> others/sbl.tex <==
\opensymdef
\newsym[Visibility]{V}{{\mathcal{V}}
\closesymdef





==> others/symb.tex <==
\opensymdef
\newsym[Visibility]{V}{{\mathcal{V}}}
\newsym[Signal]{S}{{\mathcal{S}}}
\closesymdef





==> publications.tex <==
\vspace{-1.5cm}
\singlespacing
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\section*{List of Publications } 
\subsection*{In Journals :}
\begin{itemize}
\item \footnotemark  {\bf Dutta, P.}, Begum, A., Bharadwaj, S., and Chengalur,
J.N. (2008). \\
 HI power spectrum  of the spiral galaxy NGC~628.\\
{\bf Monthly Notices of Royal Astronomical Society}, 384, L34–L37. 

\item Roy, N., Bharadwaj, S., {\bf Dutta, P.}, and Chengalur,
 J.N. (2009). \\
Magnetohydrodynamic turbulence in supernova remnants.\\
{\bf Monthly Notices of Royal Astronomical Society}, 393, L26–L30.

\item \footnotemark[\value{footnote}]  {\bf Dutta, P.}, Begum, A.,
  Bharadwaj, S., and Chengalur, J.N. (2009).\\
The scale-height of NGC~1058 measured from its HI power spectrum.\\
{\bf Monthly Notices of Royal Astronomical Society}, 397, L60–L63. 

\item \footnotemark[\value{footnote}] {\bf Dutta, P.}, Begum, A.,
  Bharadwaj, S., and Chengalur, J.N. (2009). \\ 
A study of interstellar medium of dwarf galaxies using HI power
spectrum analysis. \\
{\bf Monthly Notices of Royal Astronomical Society}, 398, 887–897.

\item Roy, N., Chengalur, J.N., {\bf Dutta, P.}, and Bharadwaj,
S. (2010).\\
H I 21 cm opacity fluctuations power spectra towards Cassiopeia A.\\
{\bf Monthly Notices of Royal Astronomical Society}, 404, L45–L49.

\item \footnotemark[\value{footnote}] {\bf Dutta, P.}, Begum, A.,
  Bharadwaj, S., and Chengalur, J.N. (2010).\\
Turbulence in the harassed galaxy NGC~4254. \\
{\bf Monthly Notices of Royal Astronomical Society}, 405, L102–L106.

\item \footnotemark[\value{footnote}] {\bf Dutta, P.}, Guha Sarkar,
  T., and Khastgir, S.P. (2010).\\  
 The effect of the $w$-term on the visibility correlation and power
 spectrum estimation. \\
{\bf Monthly Notices of Royal Astronomical Society}, L79+. 
%doi:10.1111/j.1745-3933.2010.00875.x.

\item {\bf Dutta, P.}, Khastgir, S.P., Roy, A. (2010).\\ 
Steiner trees and spanning trees in six-pin soap films. \\
{\bf American Journal of Physics}, 78, 215-221.
\end{itemize}
\footnotetext{\, \, \, Used for the present thesis}
\newpage
\subsection*{In Proceedings :}

\begin{itemize}
\item Roy, N., Bharadwaj, S., {\bf Dutta P.}, and Chengalur,
  J. N. (2009)\\ 
MHD turbulence in supernova remnants. \\
{\bf Proceeding of the 27th Meeting of the ASI in BASI, 2009}

\item {\bf Dutta, P.}, Begum, A., Bharadwaj, S., and Chengalur,
  J.N. (2009).\\
Probing Turbulence in the Interstellar Medium of Galaxies.\\
{\bf Astronomical Society of the Pacific Conference Series}, volume 407, 83

\item Roy, N., Chengalur, J.N., Bharadwaj, S., and {\bf Dutta, P.}
  (2009).\\
Turbulence in Cold Neutral ISM and in Supernova Remnants.\\
{\bf Astronomical Society of the Pacific Conference Series}, volume 407, 272
\end{itemize}

\subsection*{In Preparation :}
\begin{itemize}
\item \footnotemark[\value{footnote}] {\bf Dutta, P.}, Begum, A.,
  Bharadwaj, S., and   Chengalur, J.N. (2009). \\ 
Probing Interstellar Turbulence in Spiral Galaxies Using HI Power
Spectrum Analysis.\\
To be submitted to {\bf Monthly Notices of Royal Astronomical
  Society}.

\item {\bf Dutta, P.}, Begum, A., Bharadwaj, S., and
  Chengalur, J.N. (2009). \\ 
Simulating HI spectral observation from a turbulent ISM.\\
To be submitted to {\bf Monthly Notices of Royal Astronomical
  Society}.

\end{itemize}
\footnotetext{\, \, \, Used for the present thesis}

\newpage


==> tempbib.tex <==
\newpage
\cite{2006THS...BA} \\
\cite{2004BASI...32..335G} \\
\cite{2002ASPC..276..295O} \\
\cite{2000MNRAS.317..199D} \\
\cite{1998A&AT...17..281C} \\
\cite{1995A&A...293..507L} \\
\cite{1993MNRAS.262..327G} \\
\cite{1991PASP..103..209G} \\
\cite{1981ApJS...46..177B} \\
\cite{1973PASP...85..579T} \\
\cite{1970ApJ...160L..27V} \\
\cite{1965ApJ...142.1398C} \\
\cite{1965PhFl....8.1385K} \\
\cite{1964SvA.....7..566I} \\
\cite{1941DoSSR..30..301K} \\
\cite{2009MNRAS.395.1558C} \\
\cite{2007AJ....134.1952P} \\
\cite{2007AJ....133.1883K} \\
\cite{2007A&A...465..431H} \\
\cite{2007A&A...463..481P} \\
\cite{2005A&A...436L..53B} \\
\cite{2005MNRAS.356.1519B} \\
\cite{2004ApJ...615....7M} \\
\cite{2004ARA&A..42..275S} \\
\cite{2004ARA&A..42..211E} \\
\cite{2004A&A...413..525B} \\
\cite{2003A&A...409..879B} \\
\cite{2003A&A...398..845P} \\
\cite{2002MNRAS.334..569H} \\
\cite{2002ApJ...575L..63C} \\
\cite{2002A&A...390L..35N} \\
\cite{2002PhRvL..88x5001C} \\
\cite{2001JApA...22..293B} \\
\cite{2001AJ....121.2706F} \\
\cite{2000ApJ...537..720L} \\
\cite{2000A&ARv..10....1K} \\
\cite{1998gaas.book.....B} \\
\cite{1996AJ....111.2280S} \\
\cite{1995ApJ...438..763G} \\
\cite{1992A&A...261..353C} \\
\cite{1992A&A...253..335K} \\
\cite{1988ARA&A..26..295W} \\
\cite{1986ApJ...310..853B} \\
\cite{1984A&A...132...20S} \\
\cite{1983A&A...122..282C} \\
\cite{1980A&A....84...75F} \\
\cite{1974ApJ...194..559S} \\
\cite{2009PhRvD..79h3538B} \\
\cite{2008MNRAS.385.2166A} \\
\cite{2007ApJ...665L..19H} \\
\cite{2007MNRAS.378..119D} \\
\cite{2006MNRAS.372L..33B} \\
\cite{2006MNRAS.366..213S} \\
\cite{2005A&A...439..921V} \\
\cite{2005ApJ...624L..93B} \\
\cite{2005AJ....129.2186W} \\
\cite{2005A&A...433L...1B} \\
\cite{2004MNRAS.352..768K} \\
\cite{2003ApJ...592..975L} \\
\cite{2003ASPC..287...81V} \\
\cite{2002ApJ...566L..49C} \\
\cite{2001ApJ...563..800B} \\
\cite{2001ApJ...548..749E} \\
\cite{2000ApJ...543..227D} \\
\cite{2000AJ....120..821F} \\
\cite{1996A&AS..119..499S} \\
\cite{1996ApJ...457..455M} \\
\cite{1995MNRAS.275..863H} \\
\cite{1993ApJ...418..113P} \\
\cite{1991ApJS...75..999B} \\
\cite{1989ASPC....6.....P} \\
\cite{1984A&A...139..317G} \\
\cite{1984BAAS...16..981L} \\
\cite{1982AJ.....87..203K} \\
\cite{1962ApJ...135..151C} \\
\cite{2009MNRAS.398..887D} \\
\cite{2009MNRAS.397L..60D} \\
\cite{2009AJ....137.4526L} \\
\cite{2009MNRAS.393L..26R} \\
\cite{2008MNRAS.384L..34D} \\
\cite{2007MNRAS.375..199G} \\
\cite{2004AJ....127.2031K} \\
\cite{2003ApJ...599.1082M} \\
\cite{2003MNRAS.341..941J} \\
\cite{2001ApJ...555L..33P} \\
\cite{2000ApJ...530..133T} \\
\cite{1999ApJ...524..887R} \\
\cite{1999ApJ...514...12W} \\
\cite{1999AJ....117..868W} \\
\cite{1998AJ....116.2916F} \\
\cite{1998A&A...332...71P} \\
\cite{1995ApJ...440..706R} \\
\cite{1994ApJ...436..144F} \\
\cite{1992nrfa.book.....P} \\
\cite{1990A&A...230...21W} \\
\cite{1980ApJ...238..510B} \\
\cite{1972ApJS...24...15R} \\
\cite{2008MNRAS.386.1667B} \\
\cite{2008MNRAS.383..809B} \\
\cite{2007ApJ...671L.113L} \\
\cite{2006ApJ...644..879E} \\
\cite{2006ApJ...643..245V} \\
\cite{2006MNRAS.365.1220B} \\
\cite{1999AJ....118..853L} \\
\cite{1999MNRAS.302..417S} \\
\cite{1998A&A...336..697S} \\
\cite{1997A&A...317..203R} \\
\cite{2005AJ....130..698B} \\
\cite{1991S&T....82Q.621D} \\
\cite{1986ApJ...301..320S} \\
\cite{2008Sci...320.1195K} \\
\cite{2007ApJ...655..144M} \\
\cite{2006ApJ...645..283F} \\
\cite{2005ApJ...622L..21M} \\
\cite{2008MNRAS.384.1544S} \\
\cite{2004A&A...427..453V} \\
\cite{2004MNRAS.349..922D} \\
\cite{2006MNRAS.369..120M} \\
\cite{2004MNRAS.353..732D} \\
\cite{2005AIPC..752..161G} \\
\cite{} \\
\cite{} \\
\cite{} \\
\cite{} \\
\cite{} \\
\cite{} \\
\cite{} \\
\cite{} \\
\cite{} \\
\cite{} \\
\cite{} \\
\cite{} \\

\newpage

